On the Theoretical Properties of the Network Jackknife

We study the properties of a leave-node-out jackknife procedure for network data. Under the sparse graphon model, we prove an Efron-Stein-type inequality, showing that the network jackknife leads to conservative estimates of the variance (in expectation) for any network functional that is invariant to node permutation. For a general class of count functionals, we also establish consistency of the network jackknife. We complement our theoretical analysis with a range of simulated and real-data examples and show that the network jackknife offers competitive performance in cases where other resampling methods are known to be valid. In fact, for several network statistics, we see that the jackknife provides more accurate inferences compared to related methods such as subsampling.

==> Discussion.tex <==
\section{Discussion}
In the present work, we have shown that the network jackknife is a versatile tool that may be used in a wide variety of situations.  For poorly understood functionals, the Network Efron-Stein inequality ensures that the jackknife produces conservative estimates of the variance in expectation. For a general class of functionals related to counts, we establish consistency of the jackknife.  Our empirical investigation is encouraging regarding the finite sample properties of the procedure, as the network jackknife outperforms subsampling in many simulation settings.  %Our simulations suggest that, for variance estimation of eigenvalues, on certain graphons, the jackknife's performance is similar to subsampling. However we also see that, for some graphons, it is in fact worse than subsampling. We intend to investigate this further both theoretically and empirically.   
